A variational proof of global stability for bistable travelling waves

We give a variational proof of global stability for bistable travelling waves of scalar reaction-diffusion equations on the real line. In particular, we recover some of the classical results by P. Fife and J.B. McLeod without any use of the maximum principle. The method that is illustrated here in the simplest possible setting has been successfully applied to more general parabolic or hyperbolic gradient-like systems.

==> Fig1.tex <==
%paperxsize: 9.000
%paperysize: 5.000
\def\point#1 #2 #3 {\rlap{\kern #1 truecm
\raise #2 truecm \hbox{#3}}}
\def\spot{{\kern
-0.2em\lower.55ex\hbox{$\bullet$}}}
\def\clap#1{{\setbox0=\hbox{#1}\dimen0
=\wd0\divide\dimen0
by 2\hskip-\dimen0\box0}}
\def\dlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise-\dimen0\box0}}
\def\ulap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise\dimen0\box0}}
\def\nlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 2\raise-\dimen0\box0}}
\smash{\hbox{
\point       0.00       0.00 {$-A$}
\point       5.65       1.40 {$1$}
\point       1.20       1.30 {$0$}
\point       1.40       4.30 {$F(u)$}
\point       7.80       1.30 {$u$}
}}


==> Fig2.tex <==
%paperxsize: 9.000
%paperysize: 5.000
\def\point#1 #2 #3 {\rlap{\kern #1 truecm
\raise #2 truecm \hbox{#3}}}
\def\spot{{\kern
-0.2em\lower.55ex\hbox{$\bullet$}}}
\def\clap#1{{\setbox0=\hbox{#1}\dimen0
=\wd0\divide\dimen0
by 2\hskip-\dimen0\box0}}
\def\dlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise-\dimen0\box0}}
\def\ulap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise\dimen0\box0}}
\def\nlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 2\raise-\dimen0\box0}}
\smash{\hbox{
\point       7.20       3.85 {$(c{-}c_\infty)t$}
\point       0.90       3.70 {$\bar y(t_1)$}
\point       2.60       3.90 {$\bar y(t_2)$}
\point       4.40       4.00 {$\bar y(t_3)$}
\point       0.10       4.40 {$y$}
\point       6.15       0.50 {$\bar y(t)$}
\point       8.00       3.25 {$t$}
}}


==> Fig3.tex <==
%paperxsize: 9.000
%paperysize: 5.000
\def\point#1 #2 #3 {\rlap{\kern #1 truecm
\raise #2 truecm \hbox{#3}}}
\def\spot{{\kern
-0.2em\lower.55ex\hbox{$\bullet$}}}
\def\clap#1{{\setbox0=\hbox{#1}\dimen0
=\wd0\divide\dimen0
by 2\hskip-\dimen0\box0}}
\def\dlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise-\dimen0\box0}}
\def\ulap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise\dimen0\box0}}
\def\nlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 2\raise-\dimen0\box0}}
\smash{\hbox{
\point       2.30       2.90 {$(c_n{-}c_\infty)t$}
\point       0.30       2.00 {$\bar y(t_1)$}
\point       2.40       1.00 {$\bar y(t_2)$}
\point       6.30       1.70 {$\bar y(t)$}
\point       0.20       4.60 {$y$}
\point       8.10       4.35 {$t$}
\point       6.90       4.35 {$t_n$}
\point       5.00       4.35 {$t_n{-}T$}
\point       6.50       -0.20 {$\bar y(t_n)$}
}}


==> Fig4.tex <==
%paperxsize: 9.000
%paperysize: 5.000
\def\point#1 #2 #3 {\rlap{\kern #1 truecm
\raise #2 truecm \hbox{#3}}}
\def\spot{{\kern
-0.2em\lower.55ex\hbox{$\bullet$}}}
\def\clap#1{{\setbox0=\hbox{#1}\dimen0
=\wd0\divide\dimen0
by 2\hskip-\dimen0\box0}}
\def\dlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise-\dimen0\box0}}
\def\ulap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 1\raise\dimen0\box0}}
\def\nlap#1{{\setbox0=\hbox{#1}\dimen0
=\ht0\divide\dimen0 
by 2\raise-\dimen0\box0}}
\smash{\hbox{
\point       2.50       2.80 {$(c_n{-}c_*)t$}
\point       0.80       2.20 {$\bar y(t_1)$}
\point       1.30       0.90 {$\bar y(t_2)$}
\point       3.10       0.40 {$\bar y(t_3)$}
\point       0.40       4.40 {$y$}
\point       6.70       0.60 {$\bar y(t_n)$}
\point       8.00       4.20 {$t$}
}}

